Single-Photon Structured Light

We present a novel structured light technique that uses Single Photon Avalanche Diode (SPAD) arrays to enable 3D scanning at high-frame rates and low-light levels. This technique, called "Single-Photon Structured Light", works by sensing binary images that indicates the presence or absence of photon arrivals during each exposure; the SPAD array is used in conjunction with a high-speed binary projector, with both devices operated at speeds as high as 20~kHz. The binary images that we acquire are heavily influenced by photon noise and are easily corrupted by ambient sources of light. To address this, we develop novel temporal sequences using error correction codes that are designed to be robust to short-range effects like projector and camera defocus as well as resolution mismatch between the two devices. Our lab prototype is capable of 3D imaging in challenging scenarios involving objects with extremely low albedo or undergoing fast motion, as well as scenes under strong ambient illumination.

==> figures/fig_10_hybrid_bch.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/figure_10_hybrid_bch.pdf}
    \caption{\textbf{Hybrid strategy mitigates scene-independent short range effects.} \textit{(Top)} BCH codes, with many frames having a minimum stripe-width of 1 pixel, are easily distorted by short-range effects arising from the projector-sensor resolution mismatch and projector defocus. \textit{(Bottom)} While the distortion is lesser at higher redundancy factors, Hybrid codes are a more effective choice.}
    \label{fig:hybrid-bch-comp}
\end{figure}

==> figures/fig_14_dlp_result.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/figure_14_dlp_result.pdf}
    \caption{\textbf{Waving cloth sequence,} captured using Hybrid $(n=63)$ at $330$ FPS. The deforming folds of the cloth can be seen clearly. Capturing a non-rigid object is particularly challenging---unless we operate at high speeds, excessive motion blur is induced.}
    \label{fig:dlp-res}
\end{figure}

==> figures/fig_7_stripe_scan_robust.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/figure_7_stripe_scan_robust.pdf}
    \caption{\textbf{Stripe scanning offers robustness to random bit flips.} The decoded outputs are close to noise-free equivalents, even with multiple bit-flips occurring. Decoding involves taking a Fourier transform of the received signal to obtain the phase delay.}
    \label{fig:stripe-robust}
    \vspace{-0.1in}
\end{figure}

==> figures/fig_8_hybrid_long_run.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\columnwidth]{figures/figure_8_hybrid_long_run.pdf}
    \caption{\textbf{Hybrid encoded Long-run Gray codes.}}
    \label{fig:stripe-robust}
\end{figure}

==> figures/fig_9_decoding_bench.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\columnwidth]{figures/figure_9_decoding_benchmark.pdf}
    \vspace{-1em}
    \caption{\textbf{Minimum Distance Decoding can be significantly faster than algebraic decoding in Single-Photon SL.} We query a $512 \times 256$ array of  codewords each encoding a $10$-bit message. We compare an algebraic method (Berkelamp-Massey \cite{berlekamp_massey}) to several MDD methods including those using exhaustive search (Numpy \cite{harris2020array}, CuPy \cite{Okuta2017CuPyA}), graph-based search (BallTree \cite{balltree_boytsov2013engineering}, NNDescent \cite{nndescent_dong2011efficient}) symbolic-tensors (KeOps \cite{keops_JMLR:v22:20-275}) and batched queries (FAISS \cite{faiss_johnson2019billion}). Benchmarks reported across various BCH encoders using a Intel-i7 8700K CPU and a NVIDIA 1080Ti GPU.}
    \label{fig:decoded-bench}
    \vspace{-0.15in}
\end{figure}


==> figures/rebuttal_high_speed_comparison.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/rebuttal_high_speed_comparison.pdf}
    \vspace{-0.2in}
    \caption{\textbf{3D reconstruction from the Phantom-v2640 vs the SPAD camera.} \textit{(left)} We simulate high-speed capture using photon arrival rates.  \textit{(right)} Read-noise dominated frames of the high-speed camera lead to poor reconstructions. For a fair comparison, we use Hybrid-255 and Hybrid-127 with complementary frames as the coding scheme for the SPAD camera and the high-speed camera respectively---requiring similar acquisition times.}
    \vspace{-0.1in}
    \label{rebutfig:hand-speed-comp}
\end{figure}

==> supplementary_sections/title.tex <==
\title{Single-Photon Structured Light\\Supplementary Material}

\author{
  Varun Sundar$\,^{\dagger}$ \quad
  Sizhuo Ma$\,^\dagger$ \quad
  Aswin C.\ Sankaranarayanan$^\ddag$ \quad
  Mohit Gupta$\,^\dagger$ \\
  {$^\dagger$ University of Wisconsin-Madison} \quad
  {$^\ddag$ Carnegie Mellon University}
}
\maketitle

==> tables/event_vs_spad.tex <==
\begin{table}[tb]
  \centering
  \caption{\textbf{Comparison of event-based vision sensors and SPAD cameras.} All information needed to reproduce an event-based sensor's output is available in a SPAD's captured photon-cube. \label{tab:event_cam_vs_spad}}
  \resizebox{0.95\columnwidth}{!}{
\begin{tabular}{p{2.5cm} p{2.5cm} p{3.5cm}}
    \toprule
    {\bf Metric} & {\bf Event-Based} & {\bf SPAD Array} \\
    \midrule
    Event density      & $10^6$ events/s~\cite{Lichtsteiner:2008} & $>10^9$ counts/s~\cite{ulku512512SPAD2019} \\
    \midrule
    Low-light & \multirow{2}{*}{Moderate} & Very High \\
    performance & & \small{(single photon-sensitivity)}\\
    \midrule
    Scene types        & Dynamic & Static + Dynamic \\
    \bottomrule
  \end{tabular}}
\end{table}
